Deep Coordination Graphs

This paper introduces the deep coordination graph (DCG) for collaborative multi-agent reinforcement learning. DCG strikes a flexible trade-off between representational capacity and generalization by factoring the joint value function of all agents according to a coordination graph into payoffs between pairs of agents. The value can be maximized by local message passing along the graph, which allows training of the value function end-to-end with Q-learning. Payoff functions are approximated with deep neural networks that employ parameter sharing and low-rank approximations to significantly improve sample efficiency. We show that DCG can solve predator-prey tasks that highlight the relative overgeneralization pathology, as well as challenging StarCraft II micromanagement tasks.

==> core/fig_starcraft.tex <==
\begin{figure}[b!]	
	\centering
	\includegraphics[width=0.6\columnwidth]{img/CG_mmm2.pdf}
	\vspace{-2mm}
	\caption{\label{fig:mmm2}
			Win rate of test episodes on the SMAC map \texttt{MMM2}.
			Both \texttt{DCG} and \texttt{DCG-V} use rank 1 approximation.}
\end{figure}


